Minimizing PLM-Based Few-Shot Intent Detectors

Recent research has demonstrated the feasibility of training efficient intent detectors based on pre-trained language model~(PLM) with limited labeled data. However, deploying these detectors in resource-constrained environments such as mobile devices poses challenges due to their large sizes. In this work, we aim to address this issue by exploring techniques to minimize the size of PLM-based intent detectors trained with few-shot data. Specifically, we utilize large language models (LLMs) for data augmentation, employ a cutting-edge model compression method for knowledge distillation, and devise a vocabulary pruning mechanism called V-Prune. Through these approaches, we successfully achieve a compression ratio of 21 in model memory usage, including both Transformer and the vocabulary, while maintaining almost identical performance levels on four real-world benchmarks.

==> latex_figures/latex_figures_analysis_4Figures.tex <==
\begin{figure*}[t]
\centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[scale=0.24]{resources/analysis_acc_vs_model_size_noVal.png}
        \caption{Model size.}
        \label{figure: analysis, Model size}
    \end{subfigure}
     % \hspace{6mm}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[scale=0.24]{resources/analysis_acc_vs_vocab_size_nearest_neighbor.png}
        \caption{Vocabulary token number.}
        \label{figure: analysis, vocabulary token number}
    \end{subfigure}
     % \hspace{6mm}
    \begin{subfigure}[t]{0.23\textwidth}
        % \includegraphics[scale=0.45]{resources/acc_isotropy.png}
        \includegraphics[scale=0.24]{resources/analysis_acc_vs_vocab_pca_dim.png}
        \caption{Embedding dimension.}
        \label{figure: analysis, word embedding dimension}
    \end{subfigure}    
    \begin{subfigure}[t]{0.23\textwidth}
        % \includegraphics[scale=0.45]{resources/acc_isotropy.png}
        \includegraphics[scale=0.24]{resources/analysis_acc_vs_aug_size_noVal.png}
        \caption{Augmentation data count.}
        \label{figure: analysis, Augmentation data number}
    \end{subfigure}    
\caption{The impact of hyper-parameters on the performance.}
\label{figure: analysis}
\end{figure*}

==> latex_figures/latex_figures_analysis_acc_vs_aug_size.tex <==
\begin{figure}[h]
\centering
    \includegraphics[width=0.47\textwidth]{resources/analysis_acc_vs_aug_size_noVal.png}
    \caption{The impact of augmentation data number on the performance.}
    \label{figure: analysis_acc_vs_aug_size}
\end{figure}

==> latex_figures/latex_figures_analysis_acc_vs_compression_ratio.tex <==
\begin{figure}[h]
\centering
    \includegraphics[width=0.47\textwidth]{resources/analysis_acc_vs_model_size_noVal.png}
    \caption{The impact of model size on the performance.}
    \label{figure: analysis_acc_vs_compression_ratio}
\end{figure}

==> latex_figures/latex_figures_analysis_acc_vs_pca_dim.tex <==
\begin{figure}[h]
\centering
    \includegraphics[width=0.47\textwidth]{resources/analysis_acc_vs_vocab_pca_dim.png}
    \caption{The impact of word embedding dimension on the performance.}
    \label{figure: analysis_acc_vs_pca_dim}
\end{figure}

==> latex_figures/latex_figures_analysis_acc_vs_vocab_size.tex <==
\begin{figure}[h]
\centering
    \includegraphics[width=0.47\textwidth]{resources/analysis_acc_vs_vocab_size_nearest_neighbor.png}
    \caption{The impact of vocabulary token number on the performance.}
    \label{figure: analysis_acc_vs_vocab_size}
\end{figure}

==> sections/related.tex <==
\section{Related works}
% \textbf{CV zero-shot KD}. In computer vision, \citet{nayak2019zero} is the first work to study zero-shot knowledge distillation. It synthesizes data according to model parameters for knowledge distillation. \citet{chen2019data} also synthesizes the data to train the teacher model, but employs GAN. \citet{micaelli2019zero} adopts an adversarial generator to generate samples on which the teacher and the student fail to match, and then use them to train the student. \citet{yoo2019knowledge} train the generator by classification loss and noise recovering loss. These works assume no access to the training data, but we assume the availability of a few data. Similar to these works, we also adopt a generator to generate the transfer set.

% \textbf{CV few-shot KD}. \citet{li2020few} is the first work showing that knowledge distillation can be effectively performed with a few samples. They incrementally distill the knowledge into the small student model in a block-wise manner, matching the number of trainable parameters with the number of samples. 

% \textbf{NLP zero-shot KD}. \citet{rashid-etal-2021-towards} adopt public corpus and adversarial training to distill teacher model into a small student model under zero-shot scenario. \citet{ma2022prompting} may be the most similar work to ours. It tackles zero-shot knowledge distillation with data generated by prompting generative PLMs. Similar to the few-shot model compression we tackle in our work, the key step is sample generation, but in this work, we assume access to a few labeled data, which is usually the practical case.

% \textbf{NLP few-shot KD}. 
Rare works have been published for few-shot knowledge distillation in natural language processing (NLP). One similar work is~\cite{sauer2022knowledge}, which aims to train a small model for few-shot intent detection. However, it assumes access to an external set of annotated intent detection data, which may not be practical. 
% In addition, it employs a sophisticated meta-learning framework, By contrast, our simple method can be applied without incurring any task-scale-wise tuning. 
Another similar work is \cite{melas2020generation}, where a large language model is fine-tuned to generate new data for knowledge distillation for several text classification tasks. However, it assumes access to 100 examples for each class, which is far more than that in few-shot intent detection~\cite{zhang-etal-2022-fine, lin2023selective}. In contrast, we adopt off-the-shelf generative PLMs without fine-tuning and further design novel techniques to prune the vocabulary.
To reduce the vocabulary size, \citet{zhao-etal-2021-extremely} introduce mixed-vocabulary pre-training to train a small student model vocabulary. \citet{kolesnikovaknowledge} studies Russian, aligning the vocabulary of the teacher model and student model during distillation. However, both of them aim to train a task-agnostic small model with the minimum vocabulary size of $5000$. In contrast, we manage to build the task-specific small vocabulary of $2000$ tokens by generative PLMs.
